Active WeaSuL: Improving Weak Supervision with Active Learning

The availability of labelled data is one of the main limitations in machine learning. We can alleviate this using weak supervision: a framework that uses expert-defined rules $\boldsymbol{\lambda}$ to estimate probabilistic labels $p(y|\boldsymbol{\lambda})$ for the entire data set. These rules, however, are dependent on what experts know about the problem, and hence may be inaccurate or may fail to capture important parts of the problem-space. To mitigate this, we propose Active WeaSuL: an approach that incorporates active learning into weak supervision. In Active WeaSuL, experts do not only define rules, but they also iteratively provide the true label for a small set of points where the weak supervision model is most likely to be mistaken, which are then used to better estimate the probabilistic labels. In this way, the weak labels provide a warm start, which active learning then improves upon. We make two contributions: 1) a modification of the weak supervision loss function, such that the expert-labelled data inform and improve the combination of weak labels; and 2) the maxKL divergence sampling strategy, which determines for which data points expert labelling is most beneficial. Our experiments show that when the budget for labelling data is limited (e.g. $\leq 60$ data points), Active WeaSuL outperforms weak supervision, active learning, and competing strategies, with only a handful of labelled data points. This makes Active WeaSuL ideal for situations where obtaining labelled data is difficult.

==> sections/6-conclusion.tex <==
Obtaining labelled data can be a difficult and time-consuming problem. We can side-step this problem using weak supervision: a framework that combines expert-defined rules $\boldsymbol{\lambda}$ into probabilistic labels $p(y|\boldsymbol{\lambda}$). However, in certain cases these rules can be imprecise or cover only parts of the problem-space, thereby leading to inaccurate probabilistic labels. To alleviate this problem, we propose Active WeaSuL: using active learning to improve the weak supervision model. 

Using both artificial data and visual relationship detection data, we have shown that Active WeaSuL results in higher performance than weak supervision by itself. Compared to active learning by itself, Active WeaSuL is given a warm start: the information from the weak labels allows our model to start from a reasonable predictive performance, which we can then improve further by collecting a small set of labelled data points. 

% Importantly, Active WeaSuL achieves its optimal performance with typically only x labelled data points, suggesting that our method can enable efficient use of expert knowledge to obtain accurately labelled data in situations where labelling is challenging and time-consuming.

Throughout this work, we have compared Active WeaSuL to the work by \citet{nashaat2019hybridization, nashaat2020wesal, nashaat2020asterisk}, who have pioneered the combination of active learning and weak supervision. In our experiments, Active WeaSuL consistently outperformed their approach. We reason that the approach of \citet{nashaat2019hybridization, nashaat2020wesal, nashaat2020asterisk} requires larger amounts of active learning iterations because it relies on corrections that mostly affect individual data points, whereas Active WeaSuL requires fewer active learning iterations because it uses the expert-labelled data to learn how to best combine the weak labels.

Active WeaSuL provides means to make efficient use of domain expert knowledge: by combining expert-defined rules (weak supervision) with small amounts of expert-labelled data (active learning), we can train supervised models in applications where obtaining labelled data is difficult.

